Implied Stopping Rules for American Basket Options from Markovian Projection

This work addresses the problem of pricing American basket options in a multivariate setting, which includes among others, the Bachelier and the Black-Scholes models. In high dimensions, nonlinear partial differential equation methods for solving the problem become prohibitively costly due to the curse of dimensionality. Instead, this work proposes to use a stopping rule that depends on the dynamics of a low-dimensional Markovian projection of the given basket of assets. It is shown that the ability to approximate the original value function by a lower-dimensional approximation is a feature of the dynamics of the system and is unaffected by the path-dependent nature of the American basket option. Assuming that we know the density of the forward process and using the Laplace approximation, we first efficiently evaluate the diffusion coefficient corresponding to the low-dimensional Markovian projection of the basket. Then, we approximate the optimal early-exercise boundary of the option by solving a Hamilton-Jacobi-Bellman partial differential equation in the projected, low-dimensional space. The resulting near-optimal early-exercise boundary is used to produce an exercise strategy for the high-dimensional option, thereby providing a lower bound for the price of the American basket option. A corresponding upper bound is also provided. These bounds allow to assess the accuracy of the proposed pricing method. Indeed, our approximate early-exercise strategy provides a straightforward lower bound for the American basket option price. Following a duality argument due to Rogers, we derive a corresponding upper bound solving only the low-dimensional optimal control problem. Numerically, we show the feasibility of the method using baskets with dimensions up to fifty. In these examples, the resulting option price relative errors are only of the order of few percent.

==> abstract.tex <==
This work addresses the problem of pricing American basket options in a multivariate setting, which includes among others, the Bachelier and the Black-Scholes models.
In high dimensions, nonlinear partial differential equation methods for solving the problem become prohibitively costly due to the curse of dimensionality.
Instead, this work proposes to use a stopping rule that depends on the dynamics of a low-dimensional Markovian projection of the given basket of assets.
It is shown that the ability to approximate the original value function by a lower-dimensional approximation is a feature of the dynamics of the system and is unaffected by the path-dependent nature of the American basket option.
Assuming that we know the density of the forward process and using the Laplace approximation, we first efficiently evaluate the diffusion coefficient corresponding to the low-dimensional Markovian projection of the basket.
Then, we approximate the optimal early-exercise boundary of the option by solving a Hamilton-Jacobi-Bellman partial differential equation in the projected, low-dimensional space.
The resulting near-optimal early-exercise boundary is used to produce an exercise strategy for the high-dimensional option,
thereby providing a lower bound for the price of the American basket option.
A corresponding upper bound is also provided.
These bounds allow to assess the accuracy of the proposed pricing method.
Indeed, our approximate early-exercise strategy provides a straightforward lower bound for the American basket option price.
Following a duality argument due to Rogers, we derive a corresponding upper bound solving only the low-dimensional optimal control problem.
Numerically, we show the feasibility of the method using baskets with dimensions up to fifty.
In these examples, the resulting option price relative errors are only of the order of few percent.

==> acknowledgments.tex <==

We thank Professors Ernesto Mordecki and Fabi\'an Crocce for their feedback which significantly improved this manuscript.
Gillis Danielsen provided much-valued practitioner's views.

==> keywords.tex <==
Basket Option, Optimal Stopping, Black-Scholes, Error bounds, Monte Carlo, Markovian Projection, Hamilton-Jabcobi-Bellman

==> macros.tex <==
% \theoremstyle{theorem}
%\newtheorem{theorem}{Theorem}[section]
%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{point}[theorem]{}
%\newtheorem{assumption}[theorem]{Assumption}


%\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
%\newtheorem{example}[theorem]{Example}
%\newtheorem{notation}[theorem]{Notation}
%\newtheorem{remark}[theorem]{Remark}
%\newtheorem{condition}{Condition}

\newcommand{\F}{\operatorname{\mathcal{F}}}
\newcommand{\iF}{\operatorname{\mathcal{F}^{-1}}}

\newcommand{\Loperator}{\mathcal{L}}
%\newcommand{\R}{\mathbf{R}}
\newcommand{\Z}{\mathbf{Z}}

\newcommand{\dd}{\, \textrm{d}}
\newcommand{\e}{\textrm{exp}}
\newcommand{\fFrequency}{ f_{\omega_0}}
\newcommand{\fQuadrature}{ f_{\Delta}}

\newcommand{\I}{\mathbf{I}}

\newcommand{\ErrorFrequency}{\mathcal{E_F}}
\newcommand{\ErrorQuadrature}{\mathcal{E_Q}}
\newcommand{\Error}{\mathcal{E}}


\newcommand{\estFrequency}{\overline {\mathcal{E}}_F}
\newcommand{\estQuadrature}{\overline {\mathcal{E}}_Q}
\newcommand{\est}{\overline {\mathcal{E}}}



\newcommand{\lx}{\mathcal{L}^{X}}
\newcommand{\ls}{\mathcal{L}^{S}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\prob}[2]{\pi_{{#1,#2}}}
\newcommand{\lam}[1]{\lambda_#1}
\newcommand{\trials}[2]{\theta_{#1,#2}}
\newcommand{\damp}{\alpha}

\newcommand{\cgmyexp}{\theta}

\newcommand{\fa}{f_{\damp}}
\newcommand{\fadisc}[1]{f_{\damp, #1}}
\newcommand{\fdisc}[1]{f_{#1}}
\newcommand{\ga}{g_{\damp}}
\newcommand{\ha}{h_{\damp}}
\newcommand{\ft}[1]{\hat{#1}}
\newcommand{\ift}[1]{\iF\left[#1\right]}
\newcommand{\Lnorm}{\textrm{L}}
\newcommand{\real}[1]{\mathrm{Re}\left[#1\right]}
\newcommand{\im}[1]{\mathrm{Im}\left[#1\right]}
\newcommand{\step}{\Delta\omega}
\newcommand{\strip}[1]{A_{#1}}
\newcommand{\pureJumpProcessConstant}{C(\nu)}

\newcommand{\cutoff}{\omega_{\mathrm{\max}}}

\newcommand{\pprob}[1]{\mathrm{P} \parent{{#1}}}

\newcommand{\fnka}{f_{\damp}^{N,\cutoff}}
\newcommand{\ftnka}{\tilde f_{\damp}^{N,\cutoff}}

\newcommand{\pnka}{\Pi_{\damp}^{N,\cutoff}}

\newcommand{\fft}[2]{\mathrm{FFT}_{{#1}} \parent{{#2} }}
\newcommand{\tol}{\epsilon_{\mathrm T}}

\newcommand{\cutoffFrequency}{\omega_{\textrm{max}}}


% Juho macros
\newcommand{\partder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\der}[1]{\partial_{ #1}}
\newcommand{\ket}[1]{\left | {#1} \right \rangle }
\newcommand{\refstate}[0]{\textbf{0}}
\newcommand{\vacket}[0]{\ket{\refstate}}
\newcommand{\vacbra}[0]{\bra{\refstate}}
\newcommand{\bra}[1]{\left \langle {#1} \right | }
\newcommand{\ketbra}[1]{\ket{#1} \bra{#1}}
\newcommand{\innerprod}[2]{\left \langle {{#1} | {#2}} \right \rangle}
\newcommand{\uket}[0]{\ket{\uparrow}}
\newcommand{\dket}[0]{\ket{\downarrow}}
\newcommand{\ubra}[0]{\bra{\uparrow}}
\newcommand{\dbra}[0]{\bra{\downarrow}}
\newcommand{\hadj}[1]{{#1}^{\dagger}}
\newcommand{\transpose}[1]{{#1}^{\mathrm{T}}}
\newcommand{\conj}[1]{{#1}^{\ast}}
\newcommand{\cosine}[1]{\mathrm{cos}\left ( {#1}\right )}
\newcommand{\sine}[1]{\mathrm{sin}\left ( {#1}\right )}
\newcommand{\cosinep}[2]{\mathrm{cos}^{#2}\left ( {#1}\right )}
\newcommand{\sinep}[2]{\mathrm{sin}^{#2}\left ( {#1}\right )}
\newcommand{\expf}[1]{\mathrm{exp}\left ( {#1}\right )}
\newcommand{\expfs}[1]{\mathrm{e}^{#1}}
\newcommand{\determinant}[1]{\mathrm{det}\left ( {#1}\right )}
\newcommand{\trace}[1]{\mathrm{Tr}\left ( {#1}\right )}
\newcommand{\parent}[1]{\left( {#1} \right)}
\newcommand{\bracket}[1]{\left [ {#1} \right ]}
\newcommand{\aver}[1]{ \left\langle  {#1}  \right\rangle }
\newcommand{\absval}[1]{\left| {#1} \right|}
\newcommand{\sset}[1]{\left\lbrace {#1} \right\rbrace }
\newcommand{\arrayh}[1]{\left[ {#1} \right] }
\newcommand{\arrayv}[1]{\transpose{\arrayh{{#1}}}}
\newcommand{\iden}[1]{\mathbf{1}_{#1}}
\newcommand{\ssum}[2]{\displaystyle\sum\limits_{#1}^{#2}}
\newcommand{\pprod}[2]{\displaystyle\prod\limits_{#1}^{#2}}
\newcommand{\commut}[2]{\left[ {#1} , {#2} \right]}
\newcommand{\acommut}[2]{\left\lbrace  {#1} , {#2} \right\rbrace }
\newcommand{\spann}[1]{\mathrm{span} \parent{{#1}}}
\newcommand{\ttrace}[2]{\mathrm{Tr}_{#1} \parent{#2}}
\newcommand{\logt}[1]{\mathrm{log_2} \parent{{#1}}}
\newcommand{\hilbert}[1]{\mathcal{H}_{{#1}}}
\newcommand{\genus}{g}
\newcommand{\gsfun}[0]{\eta_{GS}}
\newcommand{\vvec}[1]{\bm{{#1}}}
\newcommand{\volavec}[0]{\vvec \sigma}
\newcommand{\vvecc}[2]{{#1}_{#2}}
\newcommand{\mmat}[1]{\mathbf{{#1}}}
\newcommand{\mmatc}[3]{{#1}_{#2 #3}}
\newcommand{\ttens}[1]{\bm{{#1}}}
\newcommand{\ddif}[0]{{\rm{d}}}
\newcommand{\kk}[0]{\vvec{k}}
\newcommand{\tsection}[1]{\newpage \section{{#1}}}
\newcommand{\grad}[0]{\nabla}
\newcommand{\divv}[0]{\nabla \dot}
\newcommand{\curl}[0]{\nabla \times}
\newcommand{\vvar}[1]{\mathrm{var} \parent{{#1}}}
\newcommand{\bigo}[1]{\mathcal O \parent{{#1}}}
\newcommand{\smallo}[1]{ o \parent{{#1}}}
\def\d{\textrm{d}}
\newcommand{\dbar}[1]{\overline{\overline{{#1}}}}

\newcommand{\startident}{\parent{\vvec x_0}}
\newcommand{\pone}[0]{\mmat{P}_1}
\newcommand{\efvec}[0]{\vvec X}
\newcommand{\efvecc}[1]{X_{#1}}
\newcommand{\eft}[1]{\efvec \parent{{#1}}}
%\newcommand{\equallaw}[0]{\stackrel{\mathclap{d}{=}}
\newcommand{\poneft}[1]{\pone \eft{{#1}}}
\newcommand{\portf}{S_1}
\newcommand{\portft}[1]{\portf \parent{#1}}
\newcommand{\pport}{\prq S^{\startident}}
\newcommand{\pportt}[1]{\pport \parent{{#1}}}
\newcommand{\efti}[2]{\vvec{F}_{#2} \parent{{#1}}}
\newcommand{\prq}[1]{\overline{{#1}}}
\newcommand{\pdrift}{\prq a^{\startident}}
\newcommand{\pvola}{\prq b^{\startident}}

\newcommand{\discount}[2]{\expf{-r \parent{{#2}-{#1}} }}
\newcommand{\discountzero}[1]{\expf{-r {#1}}}
\newcommand{\discountzeroreverse}[1]{\expf{r {#1}}}
\newcommand{\discountshort}[2]{\expfs{-r \parent{{#2}-{#1}} }}
\newcommand{\discountzeroshort}[1]{\expfs{-r {#1}}}
\newcommand{\discountzeroshortreverse}[1]{\expf{r {#1}}}

\newcommand{\stoptimeb}[0]{{\prq \tau}^\dagger }
\newcommand{\atime}[0]{q}
\newcommand{\btime}[0]{p}
\newcommand{\gmartingale}[0]{R}
\newcommand{\clockdens}[0]{\psi}

\newcommand{\pra}[0]{\prq{\vvec a}}
\newcommand{\prb}[0]{\prq{\vvec b}}
\newcommand{\bbt}[0]{{\mmat{b} \transpose{\mmat{b}}}}
\newcommand{\pbbt}[0]{\pone \bbt \transpose{\pone}}

\newcommand{\cost}[1]{C_{\mathrm{#1}}}
\newcommand{\jpar}[1]{\footnote{\color{blue} {#1} - J}}
\newcommand{\addressedpar}[2]{\footnote{{\color{red} {#1}} { \color{blue} {#2} -J}}}

\newcommand{\qt}[0]{\tilde q}
%\newcommand{\e}[1]{\times 10^{#1}}
\newcommand{\mathoper}[1]{{\mathop{\mathrm{{#1}}}}}
\newcommand{\supremum}[1]{\mathop{\mathrm{sup}}_{{#1}}}
\newcommand{\nnorm}[2]{\absval{\absval{{#1}}}_{#2}}
%\newcommand{\problem}[1]{\newpage \section*{{#1}}}
\newcommand{\hittime}[0]{\sigma_{\bar{\mathcal E}}}
\newcommand{\probb}[1]{\mathrm{P} \parent{{#1}}}
\newcommand{\expp}[1]{\mathrm{E} \bracket{{#1}}}
\newcommand{\varr}[1]{\mathrm{V} \parent{{#1}}}

\newcommand{\kaustaddress}[0]{King Abdullah University of Science and Technology, Thuwal, Kingdom of Saudi Arabia}
\newcommand{\indicatorfun}[3]{\mathbf{1}_{[{#1},{#2}]} \parent{{#3}}}
\newcommand{\indicator}{\mathbf{1}}
\newcommand{\binaryg}[1]{g_{\mathrm{bin}} \parent{#1}}
\newcommand{\binaryf}[1]{f_{\mathrm{bin}} \parent{#1}}
\newcommand{\fbinaryf}[1]{\hat{f}_{\mathrm{bin}} \parent{#1}}

\newcommand{\callg}[1]{g_{\mathrm{call}} \parent{#1}}
\newcommand{\fcallg}[1]{\hat{g}_{\mathrm{call}} \parent{#1}}
\newcommand{\fcallga}[1]{\hat{g}_{\mathrm{call}, \damp} \parent{#1}}
\newcommand{\fcallf}[1]{\hat{f}_{\mathrm{call}} \parent{#1}}
\newcommand{\fcallfa}[1]{\hat{f}_{\mathrm{call}, \damp} \parent{#1}}


\newcommand{\evaldiff}[3]{{\left [ {#1} \right ]}_{#2}^{#3}} 

%%% for the merton case
\newcommand{\sj}{\sigma_{\mathrm{jump}}}
\newcommand{\rj}{r_{\mathrm{jump}}}


%% I always forget the correct spelling
\newcommand{\levy}{L\'evy\  }
\newcommand{\ito}{It\^o\  }
%%

\newcommand{\rz}{\R - \sset{0}}



==> modapp.tex <==

\section{Laplace approximation}
\label{sec:alternates}

The Taylor expansion of the integrands in equation \eqref{eq:laplaceIntegral} can be done in various ways, and we discuss and illustrate some natural choices here. For the test case, let us consider the equal-volatility, equal weight non-correlated two-dimensional Black-Scholes model with $r = 0$ and
\begin{align*}
\pone =& [1,1], 
\\
\mmat \Sigma =& \mathoper{diag} \parent{ \transpose{[\sigma , \sigma]}},
\\
\eft 0 =& \transpose{[100,100]},
\end{align*}
with the volatility, $\sigma=0.1$.
For such a simple test case, we can evaluate the relevant expansion by hand. For a high-dimensional model, we need to resort to quadratures or Monte Carlo.

Fixing the portfolio value to $\poneft 0$, the relevant unimodal integrands in terms of the natural price of the second asset $s_2$ are given as
\begin{equation}
f_1 \parent{s_2}=
\frac{\expf{
-\frac{\parent{\mathoper{log} \parent{2- \frac{s_2}{100}}}^2}{2 \sigma^2}
-\frac{\parent{\mathoper{log} \frac{s_2}{100}}^2}{2 \sigma^2}
+ 2\mathoper{log} 
\sigma
+ \mathoper{log}
\parent{
s_2^2 - 400s^2 +40000
}
- \mathoper{log} \parent{200-s_2}
- \mathoper{log} s_2
}
}{2 \pi \sigma^2}
\label{eq:volatilityInPrice}
\end{equation}
for the numerator and 
\begin{align}
\tilde f_1 \parent{s_2}
\frac{\expf{
-\frac{\parent{\mathoper{log} \parent{2- \frac{s_2}{100}}}^2}{2 \sigma^2}
-\frac{\parent{\mathoper{log} \frac{s_2}{100}}^2}{2 \sigma^2}
- \mathoper{log} \parent{200-s_2}
- \mathoper{log} s_2
}
}{2 \pi \sigma^2}
\label{eq:densityInPrice}
\end{align}
for the denominator. Alternatively, we can express the integrals in terms of log-price $x_2 = \mathoper{log} \frac{s_2}{100}$,
\begin{align}
f_2 \parent{x_2}
=
\frac{
- \frac{\parent{\mathoper{log} \parent{2- \expfs{x_2}}}^2}{2 \sigma^2}
- \frac{x_2^2}{2 \sigma^2}
+ 2 \mathoper{log} \sigma
+ \mathoper{log} \parent{2 \expfs{2 x_2} - 4 \expfs{x_2} + 4}
- \mathoper{log} \parent{2-\expfs{x_2}}
- x_2
}{2 \pi \sigma^2}
\label{eq:volatilityInLogPrice}
\end{align}
for the numerator and
\begin{align}
\tilde f_2 \parent{x_2}
=
\frac{
- \frac{\parent{\mathoper{log} \parent{2- \expfs{x_2}}}^2}{2 \sigma^2}
- \frac{x_2^2}{2 \sigma^2}
- \mathoper{log} \parent{2-\expfs{x_2}}
- x_2
}{2 \pi \sigma^2}
\label{eq:densityInLogPrice}
\end{align}
for the denominator. With these definitions we have the unit-time projected volatility
\begin{align*}
\parent{\pvola}^2 \parent{1,200} = \frac{ \int_{\mathbb R} f_1 \parent{s_2} \ddif s_2}{\int_{\mathbb R} \tilde f_1 \parent{s_2} \ddif s_2} = \frac{\int_{\mathbb R} f_2 \parent{x_2} \ddif x_2}{\int_{\mathbb R} f_2 \parent{x_2} \ddif x_2}.
\end{align*}

The integrands $f_1$, $\tilde f_1$ and their respective second-order approximations of the form $\expf{\eta+\kappa \parent{z_2-z^*}^2}$ are illustrated in Figure \ref{fig:laplace1} for the price expansion and in Figure \ref{fig:laplace2}, log-price respectively.

\begin{figure}
\begin{center}
\begin{minipage}{150mm}
\subfigure[]{
\resizebox*{7cm}{!}{
\input{./lap1d_a_1490612491.tikz}
}
\label{fig:laplacePriceDens}
}
\hspace{5 mm}
\subfigure[]{
\resizebox*{7cm}{!}{
\input{./lap1v_a_1490612491.tikz}
}
\label{fig:laplacePriceVol}
}
\caption{Functions $f_1$ of \eqref{eq:densityInPrice} (\ref{fig:laplacePriceDens}) and $\tilde f_1$ of \eqref{eq:volatilityInPrice} (\ref{fig:laplacePriceVol}) in blue and their respective approximations based on the second-order Taylor expansions of their logarithms in dashed red.
\label{fig:laplace1}
}
\end{minipage}
\end{center}
\end{figure}

\begin{figure}
\begin{center}
\begin{minipage}{150mm}
\subfigure[]{
\resizebox*{7cm}{!}{
\input{./lap2d_a_1490612491.tikz}
}
\label{fig:laplacelPriceDens}
}
\hspace{5 mm}
\subfigure[]{
\resizebox*{7cm}{!}{
\input{./lap2v_a_1490612491.tikz}
}
\label{fig:laplacelPriceVol}
}
\caption{Functions $f_2$ of \eqref{eq:densityInLogPrice} (\ref{fig:laplacelPriceDens}) and $\tilde f_2$ of \eqref{eq:volatilityInLogPrice} (\ref{fig:laplacelPriceVol}) in blue and and their respective approximations based on the second-order Taylor expansions of their logarithms in dashed red.
\label{fig:laplace2}
}
\end{minipage}
\end{center}
\end{figure}

\begin{samepage}
The approximations are given as
\begin{align*}
2 \pi \sigma^2 f_1 \parent{s_2} \approx & \expf{2 \mathoper{log} \sigma - \parent{\frac{1}{100^2 \sigma^2}+\frac{2}{100^2}} \parent{s_2-100}^2},
\\
2 \pi \sigma^2 \tilde f_1 \parent{s_2} \approx & \expf{- 2 \mathoper{log} 200 - \parent{\frac{1}{100^2 \sigma^2}+\frac{1}{100^2}} \parent{s_2-100}^2}, 
\\
2 \pi \sigma^2 f_2 \parent{x_2} \approx & \expf{ 2\mathoper{log} \sigma + \mathoper{log} 200  - \parent{\frac{1}{\sigma^2}+2} x_2^2},
\\
2 \pi \sigma^2 \tilde f_2 \parent{x_2} \approx & \expf{- \parent{\frac{1}{\sigma^2}+1} x_2^2}
,
\end{align*}
giving for both approximations
\begin{align*}
\tilde b_1^2 \parent{1,100} = \tilde b_2^2 \parent{1,100} = 20000 \sigma^2 
\sqrt{\frac{1 + 2 \sigma^2}{1+ \sigma^2}} \approx 200.99.
\end{align*}
In contrast, with quadrature, we get a reference value of $200.98$, giving a close agreement with the Laplace-approximated value.

%Third approximation scheme can be given by approximating the density with a normal or log-normal density, expanding the argument in the exponent of either equation \eqref{eq:densityInPrice} or \eqref{eq:densityInLogPrice}.
%If a polynomial expression for the volatility term $\pbbt \parent{\vvec x \parent{\vvec z}}$ in equation \eqref{eq:laplaceIntegral} is available, one may then use a moment formula to solve the relevant integral
\end{samepage}
